Automated Evolution of Feature Logging Statement Levels Using Git Histories and Degree of Interest

Logging -- used for system events and security breaches to describe more informational yet essential aspects of software features -- is pervasive. Given the high transactionality of today's software, logging effectiveness can be reduced by information overload. Log levels help alleviate this problem by correlating a priority to logs that can be later filtered. As software evolves, however, levels of logs documenting surrounding feature implementations may also require modification as features once deemed important may have decreased in urgency and vice-versa. We present an automated approach that assists developers in evolving levels of such (feature) logs. The approach, based on mining Git histories and manipulating a degree of interest (DOI) model, transforms source code to revitalize feature log levels based on the "interestingness" of the surrounding code. Built upon JGit and Mylyn, the approach is implemented as an Eclipse IDE plug-in and evaluated on 18 Java projects with $\sim$3 million lines of code and $\sim$4K log statements. Our tool successfully analyzes 99.22% of logging statements, increases log level distributions by $\sim$20%, and increases the focus of logs in bug fix contexts $\sim$83% of the time. Moreover, pull (patch) requests were integrated into large and popular open-source projects. The results indicate that the approach is promising in assisting developers in evolving feature log levels.

==> Makefile <==
PAPER=paper
all:
	latexmk -pdf -shell-escape $(PAPER)
automated:
	latexmk -pdf -shell-escape -interaction=nonstopmode $(PAPER)
continuous:
	latexmk -pdf -pvc -shell-escape $(PAPER)
preview: all
	gio open $(PAPER).pdf
clean:
	latexmk -C $(PAPER)
	rm -rf _minted-*
	rm -f *.aux *.log *.bbl *.blg *.dvi *.synctex.gz *.out *.fdb_latexmk \
		*.fls *.nav *.toc *.snm *.spl *.vtc *.pyg *.vrb *.bcf *.run.xml *.tdo \
		*-blx.bib
	rm -rf $(PAPER)
test: automated check
check:
	chktex -xH -n 6 $(PAPER).tex 2> /dev/null | tee lint.out
html: all
	rm -rf $(PAPER)/
	latex2html -split 0 $(PAPER)
preview-html: html
	gio open $(PAPER)/index.html


==> background.tex <==
\section{Background}\label{sec:background}

\todoRKi{This should be in \cref{sec:approach}.}

\subsection{Eclipse Mylyn plugin}

\todoRKi{This section title is too technology-specific. You would never have this in a conference paper. It is fine for a tool paper.}

Our research approach reads DOI values of program elements through Mylyn. Mylyn is a task and application lifecycle management plugin in Eclipse~\cite{mylynK}. It assigns a real number to each program element (a method, a source file etc.) by evaluation of interaction events during an active task period. That real number is a representation of degree of developers' interests, and is named as ``DOI value''. Developers create a Mylyn task. They can add modify the task title and  When the task is active, all interaction events between developers and program elements could be recorded by Mylyn.

The sort of interaction events~\cite{mylyn} are listed below:
\begin{itemize}
  \item Selection: user select elements
  \item Edit: edit text in the editor
  \item Command: commands and actions invoked via buttons, menus, and keyboard shortcuts
  \item Preference: workbench preference changes
  \item Prediction: elements determined by Active Search
  \item Propagation: elements determined to be structurally related
  \item Manipulation: operation on DOI directly
  \item Attention: interaction with a task, used for the meta-context.

\end{itemize}

Mylyn drives task context from the sequence of interaction events~\cite{Kersten2006}. Task context is a graph whose elements are program elements and the edges are the relationships of elements. 

\subsection{DOI model}

DOI model is core model of Mylyn. The Mylyn's DOI model describes the interests of the code elements which are relevant to the task at hand~\cite{Kh2017}. DOI value does not only represents how developers pay attention to a program element frequently, but also show how they focus on the element recently. DOI model is a balancing model. When it increases the DOI value of a program elements through analyzing an interaction event, it could decrease the DOI value of other program elements which are not involved by the event in the task context. The operation for decreasing DOI value is named ``decay''. 

DOI values are highly tied to tasks. Each event in the task context could affect the DOI values for relevant Java code elements. The DOI value could change after the developers switch tasks, e.g.,  if a developer is working on a particular task, code elements in their project have a particular value tied to that particular test. Once they switch tasks, which is a central notion in their work, the DOI values associated with the project may change.

\subsection{Git and JGit}

%todo: what is commit
%todo: what is diff

Git is an open-source distributed version control system~\cite{git}. Git takes a picture on the files it tracks if these files have some changes. Each time developers modify file, they could make a commit and pushed the commit to the remote repository. A commit is used to store file changes for a certain version. It has its index (sha-1) to unqiuely identify itself. It also has a timestamp for the time when it is pushed. A commit has two revisions of files. One revision is old revision before modifications, the other one is new revision after modifications. Diff is file differences between two revisions of files, so the diff of a commit is the file differences between the old and new revisions. In each file, diffs for a file are composed of several hunk. Hunk is a pair of text blocks. One text block is the text deleted in first revision of file, and the other of them is the text added in the second revision of file. The hunk shows a text block change in a file. Hunk is not the samllest unit for file differences. Each hunk could contain several edits. Edit is similar as hunk, but it is always small.


JGit is a lightweight Java library of Git version control system. Developers could access repositories, read Git commits and so on through Java APIs it provides. JGit stores diffs at file level. Each file diff is store in \javainline{DiffEntry}. Every object of \javainline{DiffEntry} has its type of changes. All types of changes are following~\cite{jgitChangeType}:

\begin{itemize}
  \item ADD\@: a file addition.
  \item DELETE\@: a file deletion.
  \item COPY\@: a file copy and keep the original one. 
  \item RENAME\@: a file rename.
  \item MODIFY\@: a file content or mode modification.
\end{itemize}


==> scratch.tex <==
We help developers rejuvenate log levels in the source code to enhance logs. Developers can be able to print critical information while ignoring insignificant information through log levels. Based on the widely used Java Logging APIs we are researching on~\cite{Oracle2018}, log levels are \javainline{ALL}, \javainline{FINEST}, \javainline{FINER}, \javainline{FINE}, \javainline{CONFIG}, \javainline{INFO}, \javainline{WARNING}, \javainline{SEVERE}, \javainline{OFF}. The ordering of log levels usually reflects how developers are interested in the software parts where their log invocations are in, e.g., the software part which includes an log invocation with log level \javainline{FINEST} gains less interests from developers than the log level \javainline{INFO}. The software part is the context of a log invocation. It could be composed of some adjacent statements, enclosing block or enclosing method. Enclosing method is the method where the log invocation locates. However, there are some special cases for log levels. In this paper, we do not consider \javainline{ALL} and \javainline{OFF}, because they are used to turn on/off logging. Besides, we should consider \javainline{CONFIG}, \javainline{WARNING} and \javainline{SEVERE} carefully. \javainline{CONFIG} could be used to record static configuration information~\cite{logger}, while \javainline{WARNING} or \javainline{SEVERE} often indicates there is potential problem or a failure for program, which needs extra attention from developers. For these special log levels above, we need to consider them prudently and separately.

Developers always have challenges to evolve log levels. The previous research indicates that developers cannot well estimate cost and benefit for each log level, so they always spend much time to adjust log levels~\cite{Chen2017}. Moreover, developers always switch their interests on different software parts. At some points, developers may focus on one software part, and select a higher log levels for the log invocations in that software part. After a period of time, the software part is no longer important, but its log levels still present significance. This case always happens. \citet{Li2017}~analyzes four famous subjects and find that only 2.9\% logging statements experience level changes after their introduction. However, developers' interests always change, i.e., log levels do not always match developers' interests. They present that log levels of logging statements developers write may not be correct or may change overtime with requirements, and it is impossible to know for sure what the correct level should be. In our paper, however, we assume that more ``interesting'' parts of a software system should have, in general, higher log levels (e.g., \ji{INFO}) that less interesting parts (e.g., \ji{FINEST}). Our assumption helps developers judge the fit of log levels.

Based on our assumption, we propose an approach to help developers automatically rejuvenate log levels by using Degree Of Interests (DOI). DOI is an model which is able to provide degree of developers' interests in program elements by evaluating interaction events between developers and program elements. The model could assign a real number to an program element. That number shows the degree that developers are interested in it. That number is computed from interaction events, e.g., a developer edits an program element. DOI is a mature model and it is also implemented in Mylyn which is a Eclipse task and application life-cycle management plugin~\cite{mylynK}. Our research tries to rejuvenate log levels through matching the DOI values of their enclosing software part. However, many developers may not use, or even may not know Mylyn. We extend our theory to all Git projects. We convert git differences to Mylyn interaction events so that our tool could read DOI value for the project without using Mylyn plugin. The tool could consistently make the transformations automatically based on new developers' activities.


==> scratch2.tex <==
\begin{listing}
	\begin{javacode}
	 if (logger.isLoggable(Level.SEVERE)) {
		logger.log(Level.SEVERE, message(context), exception);
	 }
	\end{javacode}
	\caption{Logging wrapping from guava}\label{lst4}
\end{listing}

We also notice some cases that need delicate consideration. In the case of Lising\ref{lst4}, the if condition has a correlation with log level, i.e., log level is determined by if condition. In this case, we should not change a log level in a logging statement.

\begin{listing}
	\begin{diffcode}
	catch (BindException e) {
		...
	-   LOGGER.log(Level.FINE, "Failed to listen to UDP port "+PORT,e);
	+   LOGGER.log(Level.WARNING, "Failed to listen to UDP port "+PORT,e);
	 }
	\end{diffcode}
	\caption{Log level changes in catch blocks from \jenkins}\label{lst5}
\end{listing}

The last case in Listing\ref{lst5} presents developers higher the log level in a catch block. \citet{Fu2014} indicates that exception types may have correlation with developers' logging decision in a catch block. In this case, we need to process them separately.



==> scratch3.tex <==
Can our tool help bring focus to buggy code?\label{rq:bugs}

\ref{rq:bugs} inquires about our tool's ability to increase buggy code focus by altering feature logging statement levels. To help potentially expose bugs, \ref{rq:bugs} assesses whether our tool increases levels of feature logging statements in the context of bug fixes (i.e., ``buggy'' contexts) and likewise decreases levels of those in contexts of non-bug fixes (non-``buggy'' contexts).

We then assessed whether our tool increased levels of feature logging statements within the proximity of bug fixes (``buggy'' contexts) and likewise decreased levels within the proximity of non-bug fixes (non-``buggy'' contexts). The idea is that problematic feature implementations may be brought into higher developer focus before the actual code fix by increasing the levels of corresponding feature logging statements and vice-versa.

---

Which logging statements are in the context of bug fixes? What does the tool do to those? We altered gitcproc to understand this.

Use gitcproc to find bug fixes that include nearby log statements for Evaluation. Would our tool have helped in this situation?

you can look at severe bugs and say a missing log here could have revealed the cause of the bug, or avoided a long fixing process.

---

Because our approach is keyed on code edit frequency and recency, it is well-suited to ideally adjust---if necessary---feature logging statement levels to bring potentially problematic (buggy) code to the forefront, possibly exposing errors.

In other words, because feature logs typically include valuable information of corresponding feature implementations (like variable values), it may be easier to see problems with those implementations in the logs.

Places where the approach did not work well were \ldots

